SOK: On the Analysis of Web Browser Security

Web browsers are integral parts of everyone's daily life. They are commonly used for security-critical and privacy sensitive tasks, like banking transactions and checking medical records. Unfortunately, modern web browsers are too complex to be bug free (e.g., 25 million lines of code in Chrome), and their role as an interface to the cyberspace makes them an attractive target for attacks. Accordingly, web browsers naturally become an arena for demonstrating advanced exploitation techniques by attackers and state-of-the-art defenses by browser vendors. Web browsers, arguably, are the most exciting place to learn the latest security issues and techniques, but remain as a black art to most security researchers because of their fast-changing characteristics and complex code bases. To bridge this gap, this paper attempts to systematize the security landscape of modern web browsers by studying the popular classes of security bugs, their exploitation techniques, and deployed defenses. More specifically, we first introduce a unified architecture that faithfully represents the security design of four major web browsers. Second, we share insights from a 10-year longitudinal study on browser bugs. Third, we present a timeline and context of mitigation schemes and their effectiveness. Fourth, we share our lessons from a full-chain exploit used in 2020 Pwn2Own competition. and the implication of bug bounty programs to web browser security. We believe that the key takeaways from this systematization can shed light on how to advance the status quo of modern web browsers, and, importantly, how to create secure yet complex software in the future.

==> ack.tex <==
\section{Acknowledgment}
\label{s:ack}


==> lessons.tex <==
\iffalse
3 big messages (actually not 3)
 - automatic tooling to improve the security quality
   - these actually worked, clusterfuzz finding quite a lot
 - vendors take several months on mitigations fixes vs really quick 
 fixing bugs; prioritization issue?

- proactive on new features's potential security issues
  e.g. jit compiler's new features?

- Replication of Chrome Browsers
  (Add this sentence) include Electron, Node.js as Services, ... 
  (V8 is being more popular); e.g. Google's JS execution services 
  and CloudFlare's js runner services
  So it's much more significant if one vulnerability is discovered.
  - data for unanimity
    - v8
    - blink
 

- we wrote some pages about architecture, security issues about them
- highlighting good things in browsers are good; 
  design mitigations works very well, etc
  As a group knowledge, billions of users are running same codebase;
  they are chance that they are mitigating together; not single instance.
  CrowdStrike says:
  if malware is found in one enterprise; they can help others by propagating
   information to others.
  If we have collective knowledge of browsers, they can help each other.

  - case study: what we want to convey there?
  jungwon: extract some sentences
- put table
- jit spray, jit overwrite: move? make a todo item

Section 3 (unresolved)
- heap mitigation; move from dom?
- add media?
- refer stats as much as possible in sections

Section 4
- (add sentence) We describe the timeline of mitigations
\fi


==> tbl/bounty.tex <==
\begin{tabular}{|l|c|c|}
\hline
    \textbf{Attack Category} 			  & \textbf{Baseline} & \textbf{\# CVEs*}  \\ 
    \hline \hline
    Sandbox escape, non-sandboxed process exploit & Up to \$15,000                        & dummy \\ \hline
    UXSS (includes Site Isolation bypass)         & Up to \$10,000                        & dummy \\ \hline
    Renderer RCE, sandboxed process exploit       & Up to \$5,000                         & dummy \\ \hline
    Security UI Spoofing                          & Up to \$3,000                         & dummy \\ \hline
    User information disclosure                   & Up to \$2,000                         & dummy \\ \hline
    Web Platform Privilege Escalation             & Up to \$1,000                         & dummy \\ \hline
    Exploitation Mitigation Bypass                & Up to \$1,000                         & dummy \\ \hline
\end{tabular}




==> tbl/bug-list.tex <==
\begin{tabular}{lllcl}
\toprule
Num. & JS Engine  & Type & Security & Status \\
\midrule
1  & ChakraCore 1.11.5 & Incorrect regular expression parsing & & Fixed \\ 
2  & ChakraCore 1.11.5 & Incorrect regular expression parsing & & Fixed \\ 
3  & ChakraCore 1.11.5 & Escaping scope due to use-after-free & \checkmark & CVE-2019-0609 \\ % StackScriptFunction.cpp_249
4  & ChakraCore 1.11.7 & Incorrect profiling during JIT compilation && Fixed \\ 
5  & ChakraCore 1.11.7 & Memory corruption in JavascriptArray & $\triangle$ & Fixed \\ % bufferOverrun
6  & ChakraCore 1.11.7\textsc{*}  & Incorrect profiled state during JIT optimization && Fixed \\ 
7  & ChakraCore 1.11.7\textsc{*}  & Inconsistent behavior between negative NaN and positive NaN && Fixed \\ 
8  & ChakraCore 1.11.7\textsc{*}  & Breaking assumption related to the size of inline segment & \checkmark & Fixed\\ 
9  & ChakraCore 1.11.8\textsc{*}  & Inconsistency in helper label annotation during JIT compilation && Fixed \\
10 & ChakraCore 1.11.9  & Writability of read-only property in class && Reported \\ % CacheOperators.inl_367
11 & ChakraCore 1.11.9  & Writability of constant variable && Reported \\ % InlineCache.inl_240 
12 & ChakraCore 1.11.9  & Incorrect behavior when overwriting previously deleted variable && Reported \\ % PathTypeHandler.cpp_3863
13 & ChakraCore 1.11.9  & Incorrect behavior when calling getter of previously deleted variable && Reported \\ % CacheOperators.cpp_178
14 & ChakraCore 1.11.9  & Type confusion between integer and double & $\triangle$ & Reported \\ % GlobOpt.cpp_12059
15 & ChakraCore 1.11.9  & Inconsistency between cached value and real value & $\triangle$ & Reported \\ % InlineCache.h_471
16 & ChakraCore 1.11.9 & Memory corruption while building bytecode & $\triangle$ & Reported \\ % BuildIRForInlinee_bufferOverRun
17 & ChakraCore 1.11.9 & Memory corruption while parsing JS code & $\triangle$ & Reported \\ % crashCloneFrom_bufferOverRun
18 & ChakraCore 1.11.9 & Memory corruption in JavascriptArray & $\triangle$ & Reported \\ % JavascriptArray.cpp_11794
19 & ChakraCore 1.11.9 & Null dereference due to wrong scope analysis & $\triangle$ & Fixed \\ % Scope.h_207
20 & ChakraCore 1.11.9  & Breaking assumption related to the size of inline segment & \checkmark & Reported \\ % JavascriptArray.cpp_11942
21 & ChakraCore 1.11.9\textsc{*} & Incorrect internal state due to misbehavior of the engine & & Fixed\textsc{\textdagger} \\ % noreturn
22 & ChakraCore 1.11.9\textsc{*} & Wrong no-return annotation for a function which has return & & Reported \\ % noreturn
23 & ChakraCore 1.11.9\textsc{*} & Out-of-bound write due to wrong JIT optimization & \checkmark & Fixed \\ % 264284966
24 & ChakraCore 1.11.9\textsc{*} & Incorrect emitted bytecode from JIT compilation & \checkmark & CVE-2019-1023 \\ % Inline.cpp_72
25 & ChakraCore 1.11.9\textsc{*} & Use-after-free during JIT compilation & \checkmark & Confirmed \\ % 5771
26 & ChakraCore 1.11.9\textsc{*} & Out-of-bound read/write due to accessing uninitialized variable during JIT compilation & \checkmark & CVE-2019-0990 \\ % Array_OOB_and_Null_Deref_latest
27 & ChakraCore 1.11.9\textsc{*} & Out-of-bound read/write due to wrong JIT optimization & \checkmark & Confirmed \\ % oob_crash
28 & ChakraCore 1.11.9\textsc{*} & Out-of-bound read/write due to wrong inlining during JIT compilation & \checkmark & Reported \\ % 491912402
\midrule
% fixed
29 & JavaScriptCore 2.24.0 & Wrong profiling during JIT optimization & $\triangle$ & WebKit 195991 \\
30 & JavaScriptCore 2.24.1 & Invalid indices stored in TypedArrays & & WebKit 197228 \\
31 & JavaScriptCore 2.24.1 & Type confusion of induction variable during JIT compilation & $\triangle$ & WebKit 197569 \\
32 & JavaScriptCore 2.24.2 & Incorrect assumption while compiling JIT bytecode & & Fixed \\ % (WebKit 196176)
33 & JavaScriptCore 2.24.2 & Incorrect type speculation during JIT compilation & & Fixed \\
34 & JavaScriptCore 2.24.2 & Wrongly yielded exception while handling another exception & & Fixed \\ % (WebKit 196305)
35 & JavaScriptCore 2.24.2 & Inconsistent behavior of garbage collector from JIT profiling & & Fixed \\
36 & JavaScriptCore 2.24.2 & Invalid state while handling character & & Fixed \\
37 & JavaScriptCore 2.24.2 & Memory corruption while parsing function & $\triangle$ & Fixed \\
38 & JavaScriptCore 2.24.2 & Memory corruption while handling slow path in JIT code & $\triangle$ & Fixed \\
39 & JavaScriptCore 2.25.1 & Type confusion due to accessing uninitialized memory region & \checkmark & CVE-2019-6XXX \\
40 & JavaScriptCore 2.25.1 & Use-after-free due to wrong garbage collection & \checkmark & CVE-2019-6XXX \\
% crashes
41 & JavaScriptCore 2.25.1 & Memory corruption while handling regular expression & $\triangle$ & Reported \\
42 & JavaScriptCore 2.25.1 & Memory corruption while creating regular expression & $\triangle$ & Reported \\
43 & JavaScriptCore 2.25.1 & Null dereference while accessing HashMap & $\triangle$ & Reported \\
44 & JavaScriptCore 2.25.1 & Memory corruption in unreachable JIT bytecode & & Reported \\
45 & JavaScriptCore 2.25.1 & Memory corruption due to race condition in concurrent JIT compilation & $\triangle$ & Reported \\

\bottomrule
\multicolumn{5}{l}{\textsc{*}Canary version of Microsoft Edge Insider} \\
\multicolumn{5}{l}{\textsc{\textdagger} This bug was reported by us and fixed, but it is still reachable by \sys}
\end{tabular}

==> tbl/cve.tex <==
\begin{tabular}{llccr}
\hline
\# & CVE \#  	  & Bug Category  	  & Browser             & Source  \\ \hline \hline
1 & CVE-2013-1234 & JIT Optimization      & Chromium		& NVD  \\ \hline
2 & CVE-2014-1234 & Data Parsing  	  & Webkit         	& NVD  \\ \hline
3 & CVE-2015-1234 & Privacy   		  & FireFox		& N/A    \\ \hline
4 & CVE-2016-1234 & JIT Optimization   	  & Chromium            & NVD  \\ \hline
5 & CVE-2017-1234 & Logic Bug		  & Edge                & NVD  \\ \hline
\end{tabular}




==> tbl/hw-based.tex <==
\begin{tabular}{ccccc}
\hline
\textbf{Attack}
  & \textbf{Chrome}
  & \textbf{Webkit}
  & \textbf{Firefox}
  & \textbf{Edge} \\
\hline\hline

\begin{tabular}[c]{@{}c@{}} \\ Meltdown,\end{tabular}
  & \begin{tabular}[c]{@{}c@{}}Disabled\\ SAB$\dagger$\end{tabular}
  & \begin{tabular}[c]{@{}c@{}}Disabled\\ SAB\end{tabular}
  & \begin{tabular}[c]{@{}c@{}}Disabled\\ SAB\end{tabular}
  & \begin{tabular}[c]{@{}c@{}}Disabled\\ SAB\end{tabular}\\
\cline{2-5}
Spectre
  & \multicolumn{4}{c}{Reduced CPU timer precision} \\
\cline{2-5}
  & \multicolumn{2}{c}{Index masking$\dagger$}
  & -
  & Index masking \\
\hline
Glitch & $\downarrow$ GPU timer & - & - & - \\
\hline
\end{tabular}

==> tbl/sandbox.tex <==
% vim: set tabstop=2 shiftwidth=2 expandtab:
\setlength{\tabcolsep}{1pt}

\begin{tabular}{c c l| >{\centering\arraybackslash}m{13pt}
  >{\centering\arraybackslash}m{13pt} >{\centering\arraybackslash}m{13pt}
  >{\centering\arraybackslash}m{13pt} >{\centering\arraybackslash}m{13pt}
  >{\centering\arraybackslash}m{13pt} >{\centering\arraybackslash}m{13pt}
  >{\centering\arraybackslash}m{13pt} >{\centering\arraybackslash}m{13pt} |
  >{\centering\arraybackslash}m{13pt} >{\centering\arraybackslash}m{13pt}
  >{\centering\arraybackslash}m{13pt} >{\centering\arraybackslash}m{13pt}
  >{\centering\arraybackslash}m{13pt} >{\centering\arraybackslash}m{13pt}
  >{\centering\arraybackslash}m{13pt} |
  >{\centering\arraybackslash}m{13pt} >{\centering\arraybackslash}m{13pt}
  >{\centering\arraybackslash}m{13pt} |
  >{\centering\arraybackslash}m{13pt} >{\centering\arraybackslash}m{13pt}
  >{\centering\arraybackslash}m{13pt}}

  % browser header row
\toprule
\multicolumn{3}{c}{}
& \multicolumn{9}{c}{Chrome}
& \multicolumn{7}{c}{Firefox}
& \multicolumn{3}{c}{Edge}
& \multicolumn{3}{c}{Safari} \\

% browser comps row
& &
& C1 & C2 & C3
& C4 & C5 & C6
& C7 & C8 & C9
& F1 & F2 & F3 & F4
& F5 & F6 & F7
& E1 & E2 & E3
& S1 & S2 & S3
\\

\midrule
  \multirow{3}{*}{Sandboxed}
    & \G Windows & \G & \G & \G   \yes & \G
    & \G \yes & \G \yes & \G \yes
    & \G  & \G \yes & \G
    & \G \yes & \G \yes & \G \yes & \G \yes
    & \G \yes & \G \yes & \G \yes
    & \G \yes & \G \yes & \G \yes
    & \G & \G & \G
    \\

    & Linux && \yes & \yes & \yes
    &  & \yes &
    &  &  &
    & \yes & \yes &  &
    &  &  &
    &  &  &
    &  &  &
    \\

    & \G macOS & \G& \G      & \G \yes & \G
    & \G \yes & \G \yes & \G \yes
    & \G \yes & \G \yes & \G
    & \G \yes & \G \yes & \G \yes & \G \yes
    & \G  & \G \yes & \G
    & \G & \G & \G
    & \G \yes & \G \yes & \G \yes
    \\

\midrule
\midrule
  \multirow{8}{*}{\shortstack{Drop of\\ privileges}}
    & Windows & Integrity$\ddagger$
    &  & U &
    & U & U & LO
    & M & LO & M
    & LO & U & U & U
    & M & LO & M
    & LO & LO & LO
    &  &  &
    \\

    & \G Windows & \G AppContainer
    & \G  & \G  & \G
    & \G  & \G  & \G
    & \G  & \G  & \G
    & \G  & \G  & \G  & \G
    & \G  & \G  & \G
    & \G \yes & \G \yes & \G \yes
    & \G  & \G  & \G
    \\

    & Windows & Access token level$\ddagger$
    &   & LT &
    & LT & LT & K
    &  & K &
    & LT & K & K &
    & NA & LT &
    &  &  &
    &  &  &
    \\

    & \G Windows & \G Hardened token
    & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes
    & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes
    & \G  & \G  & \G
    & \G  & \G  & \G
    \\

    & Windows & Job level$\ddagger$
    & & D &
    & D & LU & LU
    &  & D &
    & D & D & D & D
    &  &  & N
    &  &  &
    &  &  &
    \\

    & \G Linux & \G NS:User*
    & \G \yes & \G IZ & \G IZ
    & \G IZ & \G \yes & \G
    & \G  & \G  & \G
    & \G \yes & \G \yes & \G  & \G
    & \G  & \G  & \G
    & \G  & \G  & \G
    & \G  & \G  & \G
    \\

  \midrule
  \multirow{8}{*}{\shortstack{Domain\\ Separation}}
    & Windows & Lockdown default DACL
    & & \yes &
    & \yes &  & \yes
    &  & \yes &
    & \yes & \yes & \yes & \yes
    &  & \yes &
    &  &  &
    &  &  &
    \\

    & \G Windows & \G Random restricting SIDs
    & \G  & \G  & \G
    & \G  & \G  & \G \yes
    & \G  & \G  & \G
    & \G \yes & \G \yes & \G \yes & \G \yes
    & \G  & \G \yes & \G
    & \G  & \G  & \G
    & \G  & \G  & \G
    \\

    & Windows & Alternate desktop
    & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes
    & \yes & \yes & \yes & \yes & \yes & \yes & \yes
    &  &  &
    &  &  &
    \\

    & \G Windows & \G Alternate window station
    & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes & \G \yes
    & \multicolumn{7}{c|}{\G }
    & \G  & \G  & \G
    & \G  & \G  & \G
    \\

    & Linux & chroot
    & \yes & \yes & \yes
    & \yes & \yes &
    &  &  &
    & \yes & \yes &
    &  &  &  &
    &  &  &
    &  &  &
    \\

    & \G Linux & \G NS:Network*
    & \G \yes & \G IZ
    & \G IZ & \G \yes & \G
    & \G  & \G  & \G
    & \G \yes & \G \yes & \G  & \G
    & \G  & \G  & \G
    & \G  & \G  & \G
    & \G  & \G  & \G & \G
    \\

    & Linux & NS:IPC
    &  &  &
    &  &  &
    &  &  &
    & \yes & \yes &  &
    &  &  &
    &  &  &
    &  &  &
    \\

    & \G Linux & \G NS:PID
    & \G \yes & \G \yes & \G \yes
    & \G \yes & \G \yes & \G
    & \G  & \G  & \G
    & \G  & \G  & \G  & \G
    & \G  & \G  & \G
    & \G  & \G  & \G
    & \G  & \G  & \G
    \\

    % & Linux & NS:PID(child)
    % & \yes & \yes & \yes
    % & \yes & \yes &
    % &  &  &
    % &  &  &  &
    % &  &  &
    % &  &  &
    % &  &  &
    % \\

  \midrule
  \multirow{5}{*}{\shortstack{Attack surface\\ reduction}}
    & \G Windows & \G Win32k.sys lockdown
    & \G  & \G \yes & \G
    & \G \yes & \G  & \G
    & \G  & \G  & \G
    & \G  & \G \yes & \G  & \G \yes
    & \G  & \G  & \G
    & \G  & \G  & \G
    & \G  & \G  & \G
    \\

    & Windows & Disable non-system font
    & & \yes &
    & \yes & \yes & \yes
    &  & \yes &
    &  &  &  &
    &  & \yes &
    &  &  &
    &  &  &
    \\

    & \G Windows & \G Hypervisor based sandboxing
    & \G  & \G  & \G
    & \G  & \G  & \G
    & \G  & \G  & \G
    & \G  & \G  & \G  & \G
    & \G  & \G  & \G
    & \G \yes & \G \yes & \G \yes
    & \G  & \G  & \G
    \\

    & Linux & System call allowlisting*
    & B & B & B
    & B & B &
    &  &  &
    & B & B &  &
    &  &  &
    &  &  &
    &  &  &
    \\

    & \G MacOS & \G System call allowlisting
    & \G & \G & \G
    & \G & \G & \G
    & \G  & \G  & \G
    & \G & \G & \G & \G
    & \G  & \G  & \G
    & \G  & \G  & \G
    & \G \yes & \G & \G
    \\

    & MacOS & \# of allowed mach services
    & & 10 &
    & 7 & 6 & 25
    & 16 & 10 &
    & 14 & 9 & 1 & 4
    &  & 55 &
    &  &  &
    & 53 & 56 & 54
    \\

    & \G MacOS & \G \# of allowed IOKits
    & \G & \G 3 & \G
    & \G 1 & \G 2 & \G 13
    & \G 0 & \G 2 & \G
    & \G 10 & \G 7 & \G 1 & \G 0
    & \G  & \G 15 & \G
    & \G  & \G  & \G
    & \G 19 & \G 18 & \G 2
    \\

\midrule
    Site Isolation$\ddagger$ & &
    &  & O &
    & O &  &
    &  &  &
    & T &  &  &
    &  &  &
    & Z & Z & Z
    &  &  &
    \\


\bottomrule

\end{tabular}

\vspace{5pt}
\setlength{\tabcolsep}{1pt}
\begin{tabular}{>{\centering\arraybackslash}m{250pt} ||
  >{\centering\arraybackslash}m{250pt}}

  \textbf{C1:} Zygote
  \textbf{C2:} Renderer
  \textbf{C3:} Storage
  \textbf{C4:} Flash
  \textbf{C5:} NaCl
  & Integrity$\ddagger$
  \textbf{U:} Untrusted, \textbf{LO:} Low, \textbf{M:}
  Medium \\

  \textbf{C6:} GPU
  \textbf{C7:} Network
  \textbf{C8:} Audio
  \textbf{C9:} Crashpad
  & Access token level$\ddagger$
  \textbf{LT:} Limited, \textbf{K:} Lockdown, \textbf{NA:} Non-Admin\\

  \textbf{F1:}  Content
  \textbf{F2:}  RDD (Media)
  \textbf{F3:}  Gecko Media Plugin
  \textbf{F4:}  Socket
  & Job level$\ddagger$
  \textbf{D:} Lockdown, \textbf{LU:} Limited User, \textbf{NE:} None \\

  \textbf{F5:}  NPAPI
  \textbf{F6:}  Flash
  \textbf{F7:}  GPU
  & NS:Network/User* 
  \textbf{IZ:} Inherited from Zygote \\

  \textbf{E1:}  Internet
  \textbf{E2:}  Flash
  \textbf{E3:}  Extension
  & System call allowlisting* 
  \textbf{B:} seccomp-BPF + Sandboxed IPC \\

  \textbf{S1:}  WebProcess
  \textbf{S2:}  GPU
  \textbf{S3:}  Network
  & Site Isolation$\ddagger$
  \textbf{O:} Origin,  \textbf{T:} Tab,  \textbf{Z:} Zone, \\

\end{tabular}


==> tbl/timer.tex <==
\begin{tabular}{l|rll}
    \toprule
    Browser     & Precision ($\mu s$) & Jitter & Landed  \\
    \hline
    \hline
    \multirow{4}{*}{Chrome}
                &                     &        & 2012-07 \\
    \cline{2-4}
                & 5                   &        & 2015-07 \\
    \cline{2-4}
                & 100                 & \yes   & 2018-01 \\
    \cline{2-4}
                & 5                   & \yes   & 2018-10 \\
    \hline
    \multirow{4}{*}{Firefox}
                &                     &        & 2012-08 \\
    \cline{2-4}
                & 20                  & \yes   & 2018-01 \\
    \cline{2-4}
                & 2000                & \yes   & 2018-03 \\
    \cline{2-4}
                & 1000                & \yes   & 2018-05 \\
    \hline
    \multirow{2}{*}{Edge}
                &                     &        & 2015-07 \\
    \cline{2-4}
                & 1000                & \yes   & 2018-03 \\
    \hline
    \multirow{3}{*}{Safari}
                &                     &        & 2014-10 \\
    \cline{2-4}
                & 100                 &        & 2015-07 \\
    \cline{2-4}
                & 1000                &        & 2018-01 \\
    \hline
    Tor Browser & 100000              & \yes   & 2015-04 \\
    \hline
\end{tabular}


==> tbl/wintoken.tex <==
\begin{tabular}{lcl}
\hline
\textbf{Integrity Level}
  & \textbf{RID Value}
  & \multicolumn{1}{c}{\textbf{Applied to}} \\
\hline\hline

Untrusted
  & 0x0000
  & JavaScript Renderers \\ \hline

Low
  & 0x1000
  & JavaScript Renderers \\ \hline

Medium
  & 0x2000
  & Broker process \\ \hline

High
  & 0x3000
  & Administrator Process \\ \hline

System
  & 0x4000
  & Critical System Service \\ \hline
\end{tabular}



